Information Obfuscation of Graph Neural Networks

While the advent of Graph Neural Networks (GNNs) has greatly improved node and graph representation learning in many applications, the neighborhood aggregation scheme exposes additional vulnerabilities to adversaries seeking to extract node-level information about sensitive attributes. In this paper, we study the problem of protecting sensitive attributes by information obfuscation when learning with graph structured data. We propose a framework to locally filter out pre-determined sensitive attributes via adversarial training with the total variation and the Wasserstein distance. Our method creates a strong defense against inference attacks, while only suffering small loss in task performance. Theoretically, we analyze the effectiveness of our framework against a worst-case adversary, and characterize an inherent trade-off between maximizing predictive accuracy and minimizing information leakage. Experiments across multiple datasets from recommender systems, knowledge graphs and quantum chemistry demonstrate that the proposed approach provides a robust defense across various graph structures and tasks, while producing competitive GNN encoders for downstream tasks.

==> privacy.tex <==

\section{Privacy Theory}
\label{sec:privacy}
\textbf{Re-structure to incorporate into the Powerful GNNs Imply Privacy Leakage Section, to keep readers motivated. Add theorems that GNNs can bring privacy concerns.}
In this section we first introduce the necessary notation used throughout the paper and briefly formalize our problem setup.

\paragraph{Notation}
We use $\data\subseteq\RR^d$ and $\ydata = \{0, 1\}$ to denote the input and output space, respectively. Similarly, $\hdata$ stands for the representation space induced from $\data$ by a feature transformation $g:\data\mapsto\hdata$. Accordingly, we respectively use $X, Y, Z$ to denote the random variables which take values in $\data, \ydata,\hdata$. In this work, we focus on $A\in\{0, 1\}$ as our binary sensitive attribute. In the context of social network, $A$ could correspond to the gender (male/female), race (white/black), or age ($\leq 40$/$>40$) of users. In this work, we assume that there is a distribution $\dist$ over $X$ where the data are sampled from. We also assume that our model is realizable. More concretely, we assume that there is a ground-truth labeling function $f_Y:\xxspace\to\{0, 1\}$ for our target task and a perfect attack function $f_A:\xxspace\to\{0, 1\}$ which extracts sensitive information $A$ from the descriptions of users. 

Given a description (input vector) of a user $\xx\in\RR^d$, the goal of a malicious adversary is to infer the sensitive attribute of the user, by also taking advantage of the structure of the network $\network$. In our context, to model the network, we use a random variable $E\in\{0, 1\}$ to denote the edge relationship between a pair of users. Alternatively, $E:\xxspace\times\xxspace\to\{0, 1\}$ could be understood as a randomized function that takes a pair of user descriptions and outputs whether they are connected in the network or not. 

A \emph{hypothesis} is a function $h:\data\to \{0, 1\}$. The prediction \emph{error} of a hypothesis $h$ w.r.t.\ the labeling function $f_Y$ under distribution $\dist$ is defined as: $\eps_\dist(h, f_Y)\defeq \Exp_{\xx\sim\dist}[|h(\xx) - f_Y(\xx)|]$. When $f$ and $h$ are binary classification functions, this definition reduces to the probability that $h$ disagrees with $f$ under $\dist$: $\Exp_{\xx\sim\dist}[|h(\xx) - f_Y(\xx)|] = \Exp_{\xx\sim\dist}[\ind(h(\xx)\neq f_Y(\xx))] = \Pr_{\xx\sim\dist}(h(\xx)\neq f_Y(\xx))$. We may drop the subscript $\dist$ for brevity when the context is clear about which distribution the data are sampled from. For two functions $g$ and $h$ with compatible domains and ranges, we use $h\circ g$ to denote the function composition $h(g(\cdot))$. Other notations will be introduced in the context when necessary.

\subsection{Problem Setup}
We consider the supervised binary classification problem as our target task. Similarly, the goal of an adversary is to infer the binary sensitive attribute $A$ given by $A = f_A(X), X\sim\dist$. Roughly speaking, our goal is to find representations $Z = g(X)$, where $g(\cdot)$ could be a randomized function, such that $Z$ is both informative about our target task of predicting $Y$ and agnostic about the sensitive attribute $A$. In order to formalize the above idea, we define $g_\sharp\dist\defeq \dist\circ g^{-1}$ to be the induced (pushforward) distribution of $\dist$ under $g$, i.e., for any event $T\subseteq\zzspace$, $g_\sharp\dist(T) \defeq \dist(g^{-1}(T)) = \dist(\{x\in\xxspace\mid g(x)\in T\})$. Hence it suffices if we could find $Z = g(X)$ such that the minimum inference error about the sensitive attribute $A$, $\inf_{h'}~\eps_\dist(h'\circ g, f_A)$, is large. At the same time, we also desire $Z=g(X)$ such that the risk of predicting $Y$ from $Z$, $\inf_h~\eps_\dist(h\circ g, f_Y)$, is small. To summarize, our overall objective could be modeled as the following minimax optimization formulation:
\begin{equation}
\min_{h, g}\max_{h'}\quad \eps_\dist(h\circ g, f_Y) - \lambda\cdot\eps_\dist(h'\circ g, f_A),
\end{equation}
where $\lambda > 0$ is a hyperparameter that trades off these two goals. 

